Co-RaL: Complementary Radar-Leg Odometry with 4-DoF Optimization and Rolling Contact

Robust and accurate localization in challenging environments is becoming crucial for SLAM. In this paper, we propose a unique sensor configuration for precise and robust odometry by integrating chip radar and a legged robot. Specifically, we introduce a tightly coupled radar-leg odometry algorithm for complementary drift correction. Adopting the 4-DoF optimization and decoupled RANSAC to mmWave chip radar significantly enhances radar odometry beyond the existing method, especially z-directional even when using a single radar. For the leg odometry, we employ rolling contact modeling-aided forward kinematics, accommodating scenarios with the potential possibility of contact drift and radar failure. We evaluate our method by comparing it with other chip radar odometry algorithms using real-world datasets with diverse environments while the datasets will be released for the robotics community. https://github.com/SangwooJung98/Co-RaL-Dataset

==> note.tex <==
What to do...

1. Single Chip Radar와 4-Dof optimization을 활용하여 3d ego-motion을 계산하는 radar velocity factor를 제안함. 
2. SPOT Quadrupedal Robot의 Joint-encoder와 Contact sensor 데이터를 활용하여 rolling motion drift를 고려한 leg velocity factor를 제안함. 
3. 복도, 계단, 등의 다양한 환경 (degenerate?)에서 취득한 데이터를 활용하여 실험을 진행 + 실험 데이터 공개
4. 코드 공개???
